Fast Classification with Sequential Feature Selection in Test Phase

This paper introduces a novel approach to active feature acquisition for classification, which is the task of sequentially selecting the most informative subset of features to achieve optimal prediction performance during testing while minimizing cost. The proposed approach involves a new lazy model that is significantly faster and more efficient compared to existing methods, while still producing comparable accuracy results. During the test phase, the proposed approach utilizes Fisher scores for feature ranking to identify the most important feature at each step. In the next step the training dataset is filtered based on the observed value of the selected feature and then we continue this process to reach to acceptable accuracy or limit of the budget for feature acquisition. The performance of the proposed approach was evaluated on synthetic and real datasets, including our new synthetic dataset, CUBE dataset and also real dataset Forest. The experimental results demonstrate that our approach achieves competitive accuracy results compared to existing methods, while significantly outperforming them in terms of speed. The source code of the algorithm is released at github with this link: https://github.com/alimirzaei/FCwSFS.

==> Alireza/Experiments.tex <==
\section{Experiments}
\label{Experiments}
In this section we compare our method with two state-of-the-art reinforce learning based methods, CWCF~\cite{cwcf} and Set-Encoding~\cite{shim2018joint}. Reinforcement learning-based active feature acquisition approaches have shown promising results in terms of accuracy on large datasets. However, these models have two significant drawbacks: The training of these models takes lots of resource and time, and these methods need huge amount of training data. These drawbacks are making them impractical for use in real-world applications. To address this issue, we have developed a simple and fast algorithm for feature selection that can be implemented efficiently and is more practical for small datasets. By leveraging the strengths of our algorithm, we can achieve accurate feature selection results without sacrificing speed and practicality.
\subsection{Experimental Setups}
\paragraph{Datasets} We conduct experiments on synthetic well-designed dataset, CUBE, MNIST and Forest.


\paragraph{\textbf{Synthetic dataset}}

In the initial phase, we assess our approach using a meticulously crafted synthetic dataset. This dataset has been purposefully designed to incorporate varying degrees of feature importance, necessitating their selection in a specific order for classification purposes. Additionally, to gauge the algorithm's capability in eliminating irrelevant features, we deliberately introduce extraneous features into the dataset.

To compare our method to other algorithms, we used SVM \cite{svm} in our evaluations this time. In order to provide a more precise evaluation of the CWCF paper algorithm, we additionally trained a model with HPC~(High-Performance Classifier). 
\begin{figure}
    \centering
    \includegraphics[width=0.65\textwidth]{images/Results/RL_Our_data.pdf}
    \caption{Our Synthetic dataset.}
    \label{fig:ours}
\end{figure}
Compared to other algorithms, figure~\ref{fig:ours} clearly demonstrates that our algorithm obtains a $\mathbf{100\%}$ accuracy rate.
Figure~\ref{fig:ours}'s results illustrate an essential point: Consistency!\\
RL-based approaches, particularly CWCF~\cite{cwcf}, are not very precise when applied to tiny datasets. This demonstrates that these complex algorithms are overfit to the tiny dataset. However, our method is consistent when data distributions change. According to Figure~\ref{fig:ours}, our algorithm, which boasts a margin of $\mathbf{20}\%$, exhibits superior accuracy compared to alternative algorithms.

\paragraph{\textbf{CUBE}} We first experiment on a synthetic dataset CUBE to see if the agent can identify a few critical features relevant to the given classification task. We use CUBE with $20$ features. We trained~\cite{shim2018joint} model precisely according to the method introduced in the Set-Encoding paper~\cite{shim2018joint}.
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{images/Results/RL_CUBE.pdf}
    \caption{CUBE with $20$ features.}
    \label{fig:cube}
\end{figure}
As shown in figure~\ref{fig:cube}, we observe that our simple and fast method can achieve better accuracy results with the same number of features.\\
An additional noteworthy observation derived from the analysis of figure~\ref{fig:cube} is that our approach exhibits a slight superiority over other reinforcement learning-based methods when the algorithm is granted access to the entirety of features. 

\paragraph{\textbf{Forest}}
On the Forest dataset, we compare our methods with those of other RL-based approaches in this part. We precisely trained their model using the~\cite{cwcf} methodology. We use $10000$ training examples to train Q~(state-action value function), C~(classifier), and \texttt{Enc}~(shared encoder). It learns via a $4$-stage Q-learning procedure. $128$ agents operate in parallel for $4$ steps every iteration.
Mini-batch updates of $128$ for 1 epoch ($4$ updates total) replace single updates. Last but not least, we have the reward as the negative classification loss $-\mathcal{L}$ from C. \texttt{Enc} is made up of a Multilayer Perceptron (MLP) with $32-32$ hidden layers that maps features to $16$-dimensional real-valued vectors and an LSTM with $16-32$ hidden layers. For the first $5000$ iterations of $\varepsilon$-greedy exploration, $\varepsilon$ is reduced linearly from $1$ to $0.1$.
\begin{figure}
    \centering
    \includegraphics[width=0.65\textwidth]{images/Results/RL_Forest.pdf}
    \caption{Forest.}
    \label{fig:forest}
\end{figure}
We find that as the number of features rises, our methods perform better than competing approaches.



\paragraph{\textbf{Computational cost comparison}}
In addition to outperforming contemporary feature selection techniques, our active feature acquisition method has a faster computational time.
\begin{table}[t]
	\centering
	\caption{Comparative analysis of the time cost of RL-based methods and our methods on three datasets. We report the average testing duration for each sample~(second).}
        \vspace{-3mm}
	\begin{tabular}{c|ccc}
		\hline
		Method & CUBE & Forest & Our Synthetic data  \\
		\hline
		RL~(CWCF)~\cite{cwcf} & $243.3$ & $272.1$ & $237.2$\\
		Set-Encoding~\cite{shim2018joint}& $47.8$ & $76.07$ & $42.5$   \\
            \hline
		  \textbf{Ours}& $\mathbf{0.0056}$ & $\mathbf{0.04}$ & $\mathbf{0.0092}$   \\
		\hline
	\end{tabular}
	\vspace{-3mm}
	\label{tab:time}
\end{table}
Table~\ref{tab:time} demonstrates that our straightforward method has a substantial time advantage.



==> Alireza/Fisher.tex <==
\section{Fisher Score}
\label{fisher}
In this section, we review Fisher score and formulating it for feature selection.

The Fisher score approach involves selecting a subset of features such that the distances between data points from different classes in the space defined by the selected features are maximized, while the distances between data points from the same class are minimized. In other words, the goal is to identify a set of features that effectively separates the different classes in the data. Specifically, if we select a subset of $m$ features, the input data matrix $\X \in \mathbb{R}^{d \times n}$ can be reduced to a matrix $\Z \in \mathbb{R}^{m \times n}$.
The computation of the Fisher Score involves the following procedure: Firstly, we calculate the matrix product between the centered between-class covariance matrix (denoted as $\si_{b}$) and the inverse of the sum of the centered within-class covariance matrix (denoted as $\si_{t}$) and a scaled identity matrix (represented by $\gamma$ times the identity matrix $\mathbf{I}$). Next, the trace of the resulting matrix is taken, which yields the value of $F(\Z)$. Mathematically, this can be written as:

\begin{equation}
F(\Z) = \mathrm{tr} \bigg\{ \left( \si_b \right) \left( \si_t + \gamma \mathbf{I} \right)^{-1}\bigg\}
\end{equation}
Let us define $\gamma$ as a positive regularization parameter. We can then express $\si_{b}$, the between-class covariance matrix, and $\si_{t}$, the total covariance matrix, as follows:
\begin{equation}
\si_{b} = \sum_{k=1}^{c}n_k(\mubold_k - \mubold)(\mubold_k - \mubold)^\top
\end{equation}
\begin{equation}
\si_{t} = \sum_{i=1}^{n}(\mathbf{z}_i - \mu)(\mathbf{z}_i - \mubold)^\top    
\end{equation}
The reduced data space is denoted as $\Z$, and $\mubold_k$ and $n_k$ are the mean vector and size of the $k^\text{th}$ class, respectively, in this space. The overall mean vector of the reduced data, denoted as $\mubold$, is calculated as the weighted average of class mean vectors. In practice, the total covariance matrix, $\si_{t}$, can be singular, so a regularization term, $\gamma \mathbf{I}$, is added to make it positive semi-definite.



==> Alireza/Notation.tex <==
\section{Preliminaries}
\label{Preliminaries}
Feature selection under supervision is a generic problem.
Let ${(\x_{i}, y_{i})}_{i=1}^{n}$ be a data set, where $\x_{i} \in \mathbb{R}^{d}$ and $y_{i} \in \{1, 2, ..., c\}$ is its class label.
Let $\X = [\x_{1}, \x_{2}, ..., \x_{n}] \in \mathbb{R}^{d\times n}$ be the data matrix where $\x_{j}$ denotes the $j\text{th}$ row of $\X$. 
We denote $\mathbf{1}$ as a vector of all ones with an appropriate length, $\mathbf{0}$ as a vector of all zeros, and $\mathbf{I}$ as an identity matrix with an appropriate size.

The problem of supervised feature selection is to find a subset of the features of size $m$ that contains the most informative features for the classification task. This can be formalized as finding a subset $\mathbf{S}$ of the feature indices $\{1, 2, ..., d\}$ such that $|\mathbf{S}| = m$ and the corresponding features provide the most discriminative information for the classification task.
